Revisiting the Time Cost Model of AllReduce

AllReduce is an important and popular collective communication primitive, which has been widely used in areas such as distributed machine learning and high performance computing. To design, analyze, and choose from various algorithms and implementations of AllReduce, the time cost model plays a crucial role, and the predominant one is the $(\alpha,\beta,\gamma)$ model. In this paper, we revisit this model, and reveal that it cannot well characterize the time cost of AllReduce on modern clusters; thus must be updated. We perform extensive measurements to identify two additional terms contributing to the time cost: the incast term and the memory access term. We augment the $(\alpha,\beta,\gamma)$ model with these two terms, and present GenModel as a result. Using GenModel, we discover two new optimalities for AllReduce algorithms, and prove that they cannot be achieved simultaneously. Finally, striking the balance between the two new optimalities, we design GenTree, an AllReduce plan generation algorithm specialized for tree-like topologies. Experiments on a real testbed with 64 GPUs show that GenTree can achieve 1.22$\times$ to 1.65$\times$ speed-up against NCCL. Large-scale simulations also confirm that GenTree can improve the state-of-the-art AllReduce algorithm by a factor of $1.2$ to $7.4$ in scenarios where the two new terms dominate.

==> 3_genmodel_eval.tex <==
%\subsection{Evaluating \model} 
\label{ssec:evalcm} 
In this section, we evaluate \model on several state-of-the-art \allr algorithms. We implement Ring \allr, RHD, \cps, and \hcps with Open MPI v4.1.1\@\cite{openmpi}. 

On our testbed, \model is parameterized by feeding Full-mesh benchmarks ranging from $N=2$ to $15$. We first test the accuracy of \model, and then take a deeper look to analyze the impact of the five terms in \model.  \par 

\input{floats/model_predictions}

We test Ring \allr, \cps, and \hcps under the scale of $12$ and $15$ processors. Hierarchical \cps is denoted by $a\times b$ meaning that the first step and the second step have fan-in degrees of $a$ and $b$, respectively. Figure \ref{fig:costmodel} shows the actual cost, \model predicted cost and the \abc model predicted cost. The results demonstrate that the error of \model is within \SI{2.6}{\percent}, which demonstrates the prediction ability of \model. As a comparison, the ($\alpha,\beta,\gamma$) model can neither estimate the cost nor select the optimal algorithm, and its error is up to \SI{19.8}{\percent}. Furthermore, the results also confirm our prediction in Section \ref{ssec:fmltmodel} that it may be beneficial to use hierarchical \allr in one single layer. \par 

\input{floats/gt_breakdown}
\input{floats/model_five_terms}

Then we break the time cost down. We set up a dedicated timer for the reduce function which involves the $\gamma$ and the $\delta$ terms (we call this \emph{calculation}). The time cost of the other three terms (the $\alpha$, $\beta$, $\varepsilon$ terms, we call this \emph{communication}) is obtained by subtracting the calculation time from the total time. We observe no obvious end-to-end latency difference before and after we set up this timer, which indicates that the timer has a negligible effect on the results. Figure \ref{fig:breakdown} shows the results. First, with the increase of the first step's fan-in degree, the calculation cost decreases monotonically. In the \SI{100}{Gbps} network, compared to Ring \allr, \cps reduces the calculation cost by \SI{61}{\percent}. This shows that the memory access overhead does exist and algorithms can benefit from reducing it. Second, the communication costs of Ring \allr and \cps are higher than others. Ring \allr has too many communication steps so the latency is high; \cps has many-to-one communications so the incast term ($\varepsilon$) emerges. With \model, all these phenomena can be reasonably explained.

In more details, Figure \ref{fig:model_five} leverages our model to analyze the impact of each term, which agrees with the break-down tests in Figure \ref{fig:breakdown}. As the sums of bandwidth and computation cost (\IE, $\beta\text{-term} + \gamma\text{-term}$) of different algorithms are the same in theory, the larger its proportion, the lower the total overhead. The other three components show a clear trade-off: with the increase of the fan-in degree, the memory I/O and latency decrease while bandwidth contention cost increases, which generates an optimal choice of $6\times2$. These results are consistent with our previous analysis, confirming the necessity of adding bandwidth contention and memory I/O terms to the existing model. \par 



%  \autoref{fig:gtvsmpi} compares the decisions of MPI and \model on different \nop. \model can characterize the difference among \algo candidates and select the optimal algorithm accurately in most scenarios, whereas MPI usually makes a wrong decision. \par 

% by demonstrating the time cost break-down of \algo on 12 processors and comparing its results with the actual experimental costs.

% As shown in \autoref{fig:breakdown}, the communication cost of \algo candidate 12 is obviously larger than other candidates, which is consistent with our previous analysis of bandwidth contention. In addition, with the increase of the first layer's width, the computation cost decreases linearly, which is in accordance with the decreasing trend of memory I/O cost. Both of these results confirm the necessity of adding bandwidth contention and memory I/O factors to the existing cost model.

% In addition, \model traverses all candidates within single-digit microseconds on typical computers. By avoiding actual attempts, the experimental overhead is largely reduced.




==> 3e_gentree_eval.tex <==
% \subsection{Evaluating \algo \allr} \label{ssec:evalgt}
In this section, we implement \algo, as shown in Algorithm~\ref{alg:gt}. Then it is evaluated on a self-implemented flow-level network simulator. This is because (1) packet-level network simulators such as NS-3 consume too much time on large networks and provide too many details; (2) it is an important contribution to create a network simulator based on \model. \par 
\input{floats/algo_impl_pscode}

\subsubsection{Physical topologies}
\input{floats/eval_gt_topo}

We set up four representative physical topologies to evaluate \algo, as shown in Figure \ref{fig:fourphytopo}.
\begin{enumerate}
    \item Single-switch network. This is a common way to build a small-scale LAN and is also an essential component for building large-scale networks. We use the instance that $24$ servers are connected to one central switch. 
    \item Symmetric hierarchical network. This is a common tree-like large network architecture. We use the instance that the root switch has 16 middle switches connected to it and each middle switch has 32 servers connected to it. There are $32\times16=512$ servers in total. 
    \item Asymmetric hierarchical network. With the gradual upgrade of data centers, they may have devices of different specifications. We use the instance that the root switch has two types of switches connected to it: (1) $8$ middle switches and each of them has $32$ servers connected to it, and (2) other $8$ middle switches and each of them has $16$ servers connected to it. There are $32\times 8 + 16\times 8=384$ servers in total. 
    \item Cross-datacenter network. Cross-data center collaboration is still a problem to be solved. It is commonly an asymmetric network whose top layer link has a low bandwidth and a high latency because it may cross the WAN. We use the instance that, (1) one data center has one root switch that has $8$ middle switches connected to it, and each of them has $32$ servers connected to it; (2) another data center has one root switch that has $8$ middle switches connected to it, and each of them has $16$ servers connected to it; (3) the two data centers' root switches are connected through one slow link. There are $32\times8 + 16\times 8=384$ servers in total.  
\end{enumerate}
The values of parameters in \model are shown in the appendix.

\subsubsection{\algo generated algorithms}
Put the above topologies into \algo, we get four customized \allr algorithms.
\begin{enumerate}
    \item On the $24$-server single-switch network, \algo uses $8\times3$ \hcps. 
    \item On the $512$-server symmetric hierarchical network, \algo uses $8\times4$ \hcps in the middle switches and \cps in the root switch.
    \item On the $384$-server asymmetric hierarchical network, \algo uses $8\times4$ \hcps in the first $8$ switches and $8\times 2$ \hcps in the last $8$ switches, and Asymmetric \cps in the root switch.
    \item On the $384$-server cross-datacenter network, \algo uses $8\times4$ \hcps in the middle switches of data center 0 and $8\times2$ \hcps in the middle switches of data center 1, and \cps in the root switches, and Asymmetric \cps between the root switches. 
\end{enumerate}

\subsubsection{Simulation results}

\dx{physical topo, logi topo, performance xx\%}

==> floats/algo_impl_pscode.tex <==
\begin{algorithm}[t]
    \caption{\algo}
    \label{alg:gt}
    \KwIn{processor $a$, data size $S$}
    % \KwOut{None}
    \BlankLine
    
    \For{$i$ in $a$.children}{
        \If{not $i$.built}{
            $i$.build($S$)\;
        }
    }
    start\_time $\leftarrow 0$\;
    \For{$i$ in $a$.children}{
        start\_time $\leftarrow$ $\max(\text{start\_time}, i\text{.finish\_time})$\;
    }
    \For{$i$ in $a$.children}{
        wait\_time $\leftarrow$ $\text{start\_time} - i\text{.finish\_time}$\;
        \If{$i.\mathrm{time\_to\_agg}(S)\leqslant\text{wait\_time}$}{
            $i$.do\_agg()\;
        }
    }
    plans $\leftarrow$ []\;
    plans $\mathbin{\text{+=}}$ all\_possible\_algo()\;
    plans $\mathbin{\text{+=}}$ all\_possible\_hier\_algo()\;
    plan\_times $\leftarrow$ []\;
    \For{$i$ in plans}{
        plan\_tiimes[$i$] $\leftarrow$ GenModel($i,S$)\;
    }
    
    best\_plan $\leftarrow$ argmin(plan\_times)\;
    min\_time $\leftarrow$ min(plan\_times)\;
    $a$.do\_scatter\_reduce(plan)\;
    $a$.built $\leftarrow$ true\;
    $a$.finish\_time $\leftarrow$ start\_time + min\_time\;
\end{algorithm}

==> floats/allr_algo_examples.tex <==
\begin{figure}[tb]
    \centering
    \begin{subfigure}[b]{0.3\linewidth}
        \centerline{\scalebox{1.2}{\xymatrix{
            *+[o][F]{1} \ar@{<->}[r]\ar@{<->}[rd] & *+[o][F]{2} \ar@{<->}[d]\ar@{<->}[ld] \\
            *+[o][F]{3} \ar@{<->}[u] & *+[o][F]{4} \ar@{<->}[l]
        }}}
        \caption{Co-located PS}
        \label{fig:ps}
    \end{subfigure}
    \begin{subfigure}[b]{0.3\linewidth}
        \centering
        \centerline{\scalebox{1.2}{\xymatrix{
            *+[o][F]{1} \ar@/^/[r] & *+[o][F]{2} \ar@/^/[d] \\
            *+[o][F]{4} \ar@/^/[u] & *+[o][F]{3} \ar@/^/[l]
        }}}
        \caption{Ring}
        \label{fig:ring}
    \end{subfigure}
    \begin{subfigure}[b]{0.36\linewidth}
        \centering
        \centerline{\scalebox{1.2}{\xymatrix@=1.2em{
            *+[o][F]{1} \ar@/^/@{<->}[r] & *+[o][F]{2} \ar@/^1em/@{<->}@<1.5em>[rr] & *+[o][F]{3} \ar@/_1em/@{<->}@<-1.5em>[ll] & *+[o][F]{4} \ar@/_/@{<->}[l]
        }}}
        \caption{RHD}
        \label{fig:rhd}
    \end{subfigure}
    \caption{Typical AllReduce algorithms}
    \label{fig:algs}
\end{figure}

==> floats/arch.tex <==
\begin{figure}[tb]
    \centerline{
    \xymatrix@=1.8em{
        *+[F]{\txt{Candidate\\Generator}} \ar[r]^{\footnotesize\txt{candidate\\ trees}} & *+[F]{\txt{\model}} \ar[r]^{\footnotesize\txt{optimal\\ algo/tree}} & *+[F]{\txt{\algo}} \\
        & *+[F]{\txt{Environment Profiler}} \ar@{.>}[u]_{\footnotesize\txt{model parameters}}
    }}
    \caption{\sys architecture}
    \label{fig:arch}
\end{figure}

==> floats/existing_algo_and_model.tex <==
\begin{table*}[tb]
    \centering
    \caption{Allreduce algorithms overhead based on existing cost model}
    \begin{tabular}{|c|c|c|c|c|c|c|}
        \hline
         Algorithm & Calc steps & Calc blocks & Comm steps & Comm data size & Comm peers & Theoretical cost \\ \hline
         Ring & $N-1$ & $2$ & $2(N-1)$ & $S/N$ & $2$ & $2(N-1)\alpha+\frac{2(N-1)S}{N}\beta+\frac{(N-1)S}{N}\gamma$\\ \hline
         RHD  & $\lceil\log N\rceil$ & $2$ & $2\lceil\log N\rceil$ & $S/2^{i}$ & $2$ & $2\lceil\log N\rceil\alpha+\frac{2(N-1)S}{N}\beta+\frac{(N-1)S}{N}\gamma$\\ \hline
         Full-mesh & $1$ & $N$ & $2$ & $S/N$ & $2(N-1)$ & $2\alpha+\frac{2(N-1)S}{N}\beta+\frac{(N-1)S}{N}\gamma$\\ \hline
    \end{tabular}
    \label{tab:ar_exist_cm}
\end{table*}

==> floats/gentree_simu_bak.tex <==
\begin{table*}[t]
    \centering
    \caption{Large-scale simulation results for GenTree. \algo means plans that generated by \algo, and \algo{*} is the special plan without data rearrangement. \dx{NOTE THAT IN-TEXT DATA NEED UPDATE}}
    \label{tab:gentreesimu}
    \footnotesize
    \begin{subtable}[t]{0.49\textwidth}
        \centering
        \caption{Single switch network (SS24/32)}
        \label{tab:singlesw}
        \begin{tabular}{c|*{3}{c}}
            \hline
            & \multicolumn{3}{c}{Time cost (s) with data size (float)} \\ \cline{2-4}
            Algorithm & \num{1e7} & \num{3.2e7} & \num{1e8} \\ \hline 
            \multicolumn{4}{c}{\textit{24 servers}} \\ \hline
            \algo & $\textbf{0.203}$ & $\textbf{0.503}$ & $\textbf{1.404}$ \\
            Ring-Allr & $1.082$ & $1.376$ & $2.288$ \\
            C-PS & $\textbf{0.203}$ & $0.562$ & $1.673$ \\ \hline
            \multicolumn{4}{c}{\textit{32 servers}} \\ \hline
            \algo & $\textbf{0.213}$ & $\textbf{0.507}$ & $\textbf{1.417}$ \\
            RHD & $0.337$ & $0.644$ & $1.593$ \\
            Ring-Allr & $1.399$ & $1.697$ & $2.617$ \\
            C-PS & $0.223$ & $0.628$ & $1.879$ \\ \hline
        \end{tabular}
    \end{subtable}
    \begin{subtable}[t]{0.49\textwidth}
        \centering
        \caption{Symmetric hierarchical network (SYM384/512)}
        \label{tab:sym}
        \begin{tabular}{c|*{3}{c}}
            \hline
            & \multicolumn{3}{c}{Time cost (s) with data size (float)} \\ \cline{2-4}
            Algorithm & \num{1e7} & \num{3.2e7} & \num{1e8} \\ \hline 
            \multicolumn{4}{c}{\textit{384 servers}} \\ \hline
            \algo & $\textbf{0.503}$ & $\textbf{1.287}$ & $\textbf{3.575}$ \\
            Ring-Allr & $2.943$ & $3.627$ & $5.742$ \\
            C-PS & $2.274$ & $7.132$ & $22.148$ \\ \hline
            \multicolumn{4}{c}{\textit{512 servers}} \\ \hline
            \algo & $\textbf{0.639}$ & $\textbf{1.627}$ & $\textbf{4.638}$ \\
            RHD & $0.896$ & $1.853$ & $4.812$ \\
            Ring-Allr & $3.571$ & $4.479$ & $7.285$ \\
            C-PS & $3.479$ & $10.989$ & $34.200$ \\ \hline
        \end{tabular}
    \end{subtable}\\[0.5em]
    \begin{subtable}[t]{0.49\textwidth}
        \centering
        \caption{Asymmetric hierarchical network (ASY384)}
        \label{tab:asym}
        \begin{tabular}{c|*{3}{c}}
            \hline
            & \multicolumn{3}{c}{Time cost (s) with data size (float)} \\ \cline{2-4}
            Algorithm & \num{1e7} & \num{3.2e7} & \num{1e8} \\ \hline 
            \algo & $\textbf{0.570}$ & $\textbf{1.593}$ & $\textbf{4.670}$ \\
            Ring-Allr & $3.043$ & $3.947$ & $6.741$ \\
            C-PS & $2.052$ & $6.421$ & $19.925$ \\
        \hline
        \end{tabular}
    \end{subtable}
    \begin{subtable}[t]{0.49\textwidth}
        \centering
        \caption{Cross-datacenter network (CDC384)}
        \label{tab:crossdc}
        \begin{tabular}{c|*{3}{c}}
            \hline
            & \multicolumn{3}{c}{Time cost (s) with data size (float)} \\ \cline{2-4}
            Algorithm & \num{1e7} & \num{3.2e7} & \num{1e8} \\ \hline 
            \algo & $\textbf{2.427}$ & $\textbf{8.299}$ & $\textbf{25.388}$ \\
            \algo{*} & $4.484$ & $13.927$ & $43.116$ \\
            Ring-Allr & $8.513$ & $17.329$ & $44.580$ \\
            C-PS & $11.890$ & $37.799$ & $117.882$ \\
        \hline
        \end{tabular}
    \end{subtable}
\end{table*}

==> floats/gt_examples.tex <==
\begin{figure*}[tb]
    \centering
    \includegraphics[width=0.95\linewidth]{floats/logitopo.pdf}
    \caption{A six-node two-layer network and its corresponding logical topology. Data on each node are split into six blocks and one tree describes how one block of data are aggregated to the root.}
    \label{fig:gt}
\end{figure*}

==> floats/hcps6.tex <==
\begin{figure}[!tb]
    \centering
    \includegraphics[width=0.74\linewidth*\real{0.92}, height=(\linewidth*\real{0.9065}*\real{0.92})]{floats/basicplan6_T.pdf}
    \caption{\algo Hierarchical \allr on a symmetric tree topology that shows in Figure \ref{fig:phytopo6} ($3\times2$). Numbers are node labels and letters are data blocks. ``Placement of swX'' refers to the placements in the basic \sr plan for the swX-local sub-tree.}
    \label{fig:hcps6}
\end{figure}

==> floats/hcps7.tex <==
\begin{figure}[!tb]
    \centering
    \includegraphics[width=0.85\linewidth*\real{0.92}]{floats/hcps7.pdf}
    \caption{\algo \sr sub-plans on the asymmetric tree topology that shows in Figure \ref{fig:phytopo7}. Numbers are node labels and letters are data blocks. ``Placement of swX'' refers to the placements in the basic \sr plan for the swX-local sub-tree. }
    \label{fig:hcps7}
\end{figure}

==> floats/logical_topo_tree_example.tex <==
\begin{figure}[t]
    \centering
    \centerline{\scalebox{1.2}{\xymatrix@=1.2em{
        && *+[o][F]{2} && \\
        & *+[o][F]{2} \ar@{--}[ur] && *+[o][F]{3} \ar@{-}[ul] & \\
        *+[o][F]{0} \ar@{-}[ur] & *+[o][F]{1} \ar@{-}[u] & *+[o][F]{2} \ar@{--}[ul] & *+[o][F]{3} \ar@{--}[u] & *+[o][F]{4} \ar@{-}[ul]
    }}}
    \caption{Example of one tree in logical topology. This describes how one block of data is aggregated from all nodes to the root.}
    \label{fig:logitreeexample}
\end{figure}

==> floats/ompi_model.tex <==
\begin{table}[tb]
    \optima\footnotesize
    \centering
    \caption{\texttt{MPI\_Allreduce} decisions of Open MPI when operation is commutative in brief.}
    \begin{tabular}{|c|c|c|c|c|c|c|c|}
        \hline
        %  \diagbox{$S$}{$N$} & $<8$ & $<16$ & $<32$ & $<64$ & $<512$ & $<4096$ \\ \hline
        %  $<\SI{8}{\byte}$ & Ring & RD & SR & SR & RB & RB \\ \hline
        %  $<\SI{64}{\byte}$ & RD & RD & SR & SR & RB & RB\\ \hline
        %  $<\SI{2048}{\byte}$ & RD & RD & RD & RHD & RB & RB\\ \hline
        %  $<\SI{8192}{\byte}$ & RD & RD & RHD & RHD & RHD & RD \\ \hline
        %  $<\SI{16384}{\byte}$ & RHD & RHD & RHD & RHD & RHD & RD\\ \hline
        %  $\geqslant \SI{16384}{\byte}$ & RHD & RHD & RHD & RHD & RHD & RHD\\ \hline
        \diagbox{$\bm{S}$}{$\bm{N}$} & $<2^2$ & $<2^3$ & $<2^4$ & $<2^9$ & $<2^{12}$ & $>$\\ \hline
        $<2^3$ & Ring & Ring & RD & RB & RB & RB\\ \hline
        $<2^4$ & RD & Ring & RD & RB & RB & RB\\ \hline
        %$<2^{11}$ & RD & RD & RD & RB & RB & RB\\ \hline
        $<2^{12}$ & RD & RD & RD & RB & SR & SR\\ \hline
        $<2^{13}$ & Ring & RD & RD & RHD & RD & SR\\ \hline
        %$<2^{14}$ & RD & RHD & RHD & RHD & RD & SR\\ \hline
        $<2^{15}$ & RD & RHD & RHD & RHD & RD & RD\\ \hline
        $<2^{17}$ & Ring & RHD & RHD & RHD & RHD & RHD\\ \hline
        $<2^{18}$ & SR & RHD & RHD & RHD & RHD & RHD\\ \hline
        $>$ & RHD & RHD & RHD & RHD & RHD & RHD\\ \hline
    \end{tabular}
    \label{tab:ompidec}
\end{table}
